PrivCirNet: Efficient Private Inference via Block Circulant Transformation

Homomorphic encryption (HE)-based deep neural network (DNN) inference protects data and model privacy but suffers from significant computation overhead. We observe transforming the DNN weights into circulant matrices converts general matrix-vector multiplications into HE-friendly 1-dimensional convolutions, drastically reducing the HE computation cost. Hence, in this paper, we propose \method, a protocol/network co-optimization framework based on block circulant transformation. At the protocol level, PrivCirNet customizes the HE encoding algorithm that is fully compatible with the block circulant transformation and reduces the computation latency in proportion to the block size. At the network level, we propose a latency-aware formulation to search for the layer-wise block size assignment based on second-order information. PrivCirNet also leverages layer fusion to further reduce the inference cost. We compare PrivCirNet with the state-of-the-art HE-based framework Bolt (IEEE S\&P 2024) and the HE-friendly pruning method SpENCNN (ICML 2023). For ResNet-18 and Vision Transformer (ViT) on Tiny ImageNet, PrivCirNet reduces latency by $5.0\times$ and $1.3\times$ with iso-accuracy over Bolt, respectively, and improves accuracy by $4.1\%$ and $12\%$ over SpENCNN, respectively. For MobileNetV2 on ImageNet, PrivCirNet achieves $1.7\times$ lower latency and $4.2\%$ better accuracy over Bolt and SpENCNN, respectively. Our code and checkpoints are available on Git Hub.

==> sec/abandon.tex <==
%  Nevertheless, \textbf{\underline{1)}} they don't reduce the number of HE multiplications. Previous works focus on reducing HE rotations since they are an order of magnitude slower than multiplications. However, we profile the latency breakdown of MobileNetV2 and BERT-Base Feed Forward Network (FFN)~\cite{} based on Bolt protocols~\cite{}. We find \textit{HE multiplications are also the latency bottleneck since the number of multiplications far exceeds the number of rotations which are highly optimized}. 
    
    % However, HE only supports linear layers of a neural network. To enable private inference of nonlinear layers, some fully homomorphic encryption (FHE)-based methods approximate activations by a square function to perform the whole secure inferences on cloud without involving the client~\cite{}. However, FHE-based methods lead to a significant accuracy drop and require expensive bootstrapping operation. While other hybrid HENNs take advantage of secure two-party computation (2PC) to get the client involved in the computation of activation layers by exchanging data between the client and the server. With the development of 2PC techniques in recent years, HE becomes the computation and communication bottleneck of hybrid HENNs inference~\cite{}. Hence, many previous works concentrate on optimizing the HE encoding methods to improve the communication and computation efficiency. These HE encoding methods can be roughly divided into two categories: \textbf{\underline{1)}} single-instruction-multiple-data (SIMD) encoding~\cite{} and \textbf{\underline{2)}} polynomial coefficient encoding~\cite{}. However, as shown in Figure~\ref{}\xts{need a figure show CTF2 and Cheetah: HE Comm/Latency, MPC Comm/Latency}, SIMD encoding suffers from massive computation due to expensive rotation operations, while coefficient encoding suffers from high communication cost due to low utilization of coefficients. Thus, the HE operations become 
    % the performance bottleneck and lead to orders of magnitude slower of HENNs than plaintexts inference. % the input vector $X$ and circulant weight matrix $W$ are first converted to frequency-domain representation by discrete Fourier transform (DFT). Then only element-wise multiplications are required to perform frequency-domain convolutions and finally we conduct inverse DFT (IDFT) to get the output vector $Y$. Hence, in a circulant vector-matrix multiplication, there are no rotations needed. However, the FHE-based method need to conduct homomorphic DFT and IDFT on encrypted data $X$ and $Y$, introducing additional computations for conversion, which could negate circulant matrices' advantages. What's worse, previous works~\cite{} utilize SIMD encoding to conduct matrix-matrix multiplications (Figure~\ref{fig:cir_intro} (a))\xts{need a blockcir figure and zoom in single one circulant GEVM} which needs to perform vector-matrix multiplications on each row of the input. This leads to a large number of rotations and thus unacceptable latency. For example,~\cite{} needs 107 seconds to perform a single three-layer network on CIFAR-10 dataset. 


    % Additionally, previous works~\cite{} have relatively huge accuracy drop when introducing circulant matrices, such as  76.5\% Top-1 accuracy on CIFAR-10 in Falcon~\cite{}. And compression ration of each layer is manually configured in~\cite{}, which will result in suboptimal performance.


% Therefore, previous works concentrate on optimizing the HE encoding methods to improve both the communication and computation efficiency. There are two mainstream encoding methods: \textbf{\underline{1)}} single-instruction-multiple-data (SIMD) encoding~\cite{} and \textbf{\underline{2)}} polynomial coefficient encoding~\cite{}. However, SIMD encoding suffers from massive computation due to expensive rotation operations. While coefficient encoding eliminate rotations, it suffers from high communication cost due to low utilization of coefficients. Recent works~\cite{ju2023neujeans,pang2023bolt} argue that it is more important to save on network communication as computations can be accelerated and parallelized such as~\cite{}. To this end,~\cite{ju2023neujeans,pang2023bolt}~propose new encoding methods which minimize the communication first and reduce a number of rotations, achieving SOTA performance. In Figure~\ref{fig:moti1}, we profile the latency breakdown of MobileNetV2 and BERT-Base Feed Forward Network (FFN)~\cite{} based on Bolt protocols~\cite{}. We find that \textbf{\underline{1)}} \textit{HE multiplications are the important latency bottleneck since the number of multiplications far exceeds the number of rotations which are highly optimized by previous works}~\cite{}. \textbf{\underline{2)}} There is still a certain amount of rotation present. Hence, HE operations are still the performance bottleneck and lead to orders of magnitude slower of HENNs than plaintext inference. 

% Another type of works optimize the network architecture to improve the efficiency of HE inference.~\cite{} reduce the cost of nonlinear layers through nonlinear operation pruning and approximation. For linear layers, structured pruning~\cite{liu2019metapruning} reduce the network volume to reduce the inference latency at the cost of huge accuracy degradation.~\cite{spencnn} reduces the number of rotations through pruning the $3\times 3,5\times 5$ convolution kernels. However, for a general matrix multiplication (GEMM) which is widely used in efficient CNNs, e.g., $1\times 1$ convolution in MobileNets and in transformer models, e.g., self-attention and FFN, there isn't a good solution to reduce the HE inference latency while maintaining high accuracy.


% \begin{wrapfigure}[11]{l}[0em]{0.5\textwidth}
%     \includegraphics[width=1.0\linewidth]{figs/intro_moti1.pdf}
%     \caption{}\label{fig:moti1}
% \end{wrapfigure}

% \begin{wrapfigure}[11]{r}[0em]{0.5\textwidth}
%     \includegraphics[width=1.0\linewidth]{figs/cir_intro.pdf}
%     \caption{\xts{all figures will be updated in the end at once!!}}\label{fig:cir_intro}
% \end{wrapfigure}

% we propose~\method~for fast HENNs inference with block circulant weight matrices. \textbf{\underline{1)}} We argue that  using block circulant transformation in the hybrid HENNs,so that DFT and iDFT can run on plaintext and its overhead can be ignored. \textbf{\underline{2)}} Furthermore, we find single circulant matrix-matrix multiplication is naturally friendly to polynomial coefficient encoding while the calculation between different circulant blocks are naturally friendly to SIMD encoding, enabling us to combine the advantages of these two encoding schemes and propose~\encode. Compared with the SOTA encoding method~\cite{ju2023neujeans}, ~\encode~can reduce the number of ciphertext-plaintext (ct-pt) multiplication by \textit{block size} times and the rotations by $\sqrt {\text{block size}} $times, while minimizing communication complexity. That means even with the block size=2,~\encode~can also achieve a performance improvement of $\sqrt{2} \sim 2 \times$. \textbf{\underline{3)}} Finally, to further improve the network accuracy, we design a HE-Aware network compression algorithm, which uses the cost of hybrid HENNs inference as a guide to determine the layer-wise block size. Our contributions can be summarized as follows.
% \begin{itemize}
%     \item 1
%     \item 2
%     \item 3
% \end{itemize}

% There mainly exist two types of HENNs: FHE~\cite{} and hybrid HENNs~\cite{}. FHE-based HENNs have huge difficulties to deal with non-linear layers. One way is to approximate the non-linear functions with polynomials~\cite{}, which introduces huge accuracy degradation and computation cost, especially the expensive bootstrapping. Others utilize Fully Homomorphic Encryption over the Torus (TFHE) to evaluate non-linear layers~\cite{}. However, both methods are several orders of magnitude slower than MPC-based methods~\cite{}, keeping them far from practical. 

% In this section, we present the technical details of~\method~framework. Figure~\ref{fig:overview} shows an overview of the~\method~framework where we co-design the private protocol and network optimization. At the protocol level, we first propose~\encode, a novel encoding method for block circulant matrix multiplication. Then, we propose InvertedResidual Fusion for MobileNetV2~\cite{} where we consecutively compute two linear layers to further reduce communication cost. At the network level, we first apply a block circulant matrix to compress the weight matrices of the neural network. Then, to improve accuracy, we propose a new Latency-Aware DNAS algorithm to search for the optimal network architecture. Finally, we propose Circulant-Aware
% Conv+BN Fusion to fuse the block circulant convolution and batch normalization layers to further reduce latency in private inference.

% \paragraph{Search algorithm}
% Intuitively, a layer that is more sensitive to errors requires a smaller block size. HAWQ-V3~\cite{yao2021hawq} use the metric $\frac{\lambda_i}{m_i}\left \|W_i^\prime-W_i \right\|^2_2$ to approximate the sensitivity of each layer in a quantized network, where $\lambda_i$ is the average eigenvalue of the Hessian of weight, $m_i$ is the number of parameters in $W_i$ and $W^\prime_i$ is the compressed weight. However, directly using this metric in block circulant HENNs results in even worse accuracy than the uniform block size, as shown in Table~\ref{}. We visualize the layer-wise sensitivity in Figure~\ref{} and find two problems: \textbf{\underline{1)}} Misleading sensitivity of block size from 1 to 2.  Different from network quantization~\cite{}, the error on weight is significant even with block size $2$ and thus there exists a huge sensitivity gap between block sizes 1 and 2. This is contrary to the fact that after fine-tuning, a uniform block size of 2 has little impact on accuracy. 
% \textbf{\underline{2)}} The sensitivity distribution between layers is chaotic. 

% To tackle these problems, we propose to delete the block size of 1 in the search space since a block size of 2 has little accuracy degradation. Then, we propose a new sensitivity metric that takes the layer input $X_i$ into account:
% \begin{equation}
%     \Omega_i = \frac{\lambda_i}{m_i}\left \|W_i^\prime X_i-W_i X_i \right\|^2_2
% \end{equation}
% This metric has smoother layer-wise sensitivity for circulant network as observed in Figure~\ref{fig:sensitivity}(b). Furthermore, we proof in Theorem~\ref{theorem:sensitivity} that this metric prefers weights with smaller variance and inputs with smaller $L_2$ norm, which in a way reveals the characteristics of circulant networks. We defer the proof to Appendix~\ref{}.

% \begin{theorem}\label{theorem:sensitivity}
%     Given a layer with input $X$, weight $W$ and circulant weight $W^\prime$, the sensitivity metric $\frac{\lambda}{m}\left \|W^\prime X-W X \right\|^2_2 \le \lambda \mathbb{E}_{j}\left[ \operatorname{var}(W_j)\right]\left \| X \right \|_2^2$, where $\operatorname{var}$ is the variance and $W_j$ is the $j$-th diagonal of $W$.
% \end{theorem}

% \begin{theorem}\label{theorem:sensitivity}
%     Given a layer with input $X$, weight $W$ and circulant weight $W^\prime$, the sensitivity metric $\frac{\lambda}{m}\left \|W^\prime -W \right\|^2_2 = \lambda \mathbb{E}_{j}\left[ \operatorname{var}(W_j)\right]$, where $\operatorname{var}$ is the variance and $W_j$ is the $j$-th diagonal of $W$.
% \end{theorem}

% However, there widely exist consecutive linear layers in neural networks that possess the potential for fusion, such as self-attention layer fusion in Bolt~\cite{}.

% In an inverted residual block, the ending is a $\operatorname{conv}$ and $\operatorname{bn}$ without a nonlinear activation function, enabling us to continue the computation of the subsequent residual addition and the next linear layer. 

% The main difficulty is we need to keep both the packing and the block size of $x_1,y_1,x_{res}$ the same to compute $\operatorname{convbn}(x_{res}+\operatorname{convbn}(x_1))$ at once. 

% \begin{wraptable}[4]{r}[0em]{0.5\textwidth}
%     \renewcommand{\arraystretch}{1}
%     \centering
%     \caption{Comparison with SpENCNN in number of rotations left.}
%     \label{tab:bsgs}
%     \resizebox{1.0\linewidth}{!}{
%     \begin{tabular}{c|c|cccc}
%     \toprule 
%     % \toprule
%     \multirow{2}{*}{Method}& \multirow{2}{*}{\makecell{Sparsity/\\ Block size}} &\multicolumn{4}{c}{Number of rotations left (\%) $\downarrow$}\\
%     \cmidrule{3-6}
%     & & MBV2& ViT& ViT-Tiny& Average\\
%     \midrule
%     \multirow{3}{*}{\makecell{SpENCNN\\ \cite{spencnn}}}& 50\% &100 &100 &100 &100\\\
%     & 75\% &99.36 &97.85 &99.26 &96.69\\
%     & 87.5\% &92.96 &97.85 &99.26 &96.69\\
%     \midrule
%     \multirow{3}{*}{\makecell{\method\\ (ours)}}& b=2 &60.98 &65.25 &61.75 &\textbf{62.66}\\
%     & b=4 &35.23 &41.92 &36.32 &\textbf{37.82}\\
%     & b=8 &21.05 &27.70 &19.02 &\textbf{22.59}\\
%     % \multirow{2}{*}{+BSGS}& $O(d_1d_2d_3/(nb))$ &$O(\sqrt{d_1^2d_2^2d_3/(bn^2)})$  &$O(d_1d_2/n)$ & $O(d_1d_3/n)$\\
%     % &48&4&0.11 MB&0.68 MB  \\
%     \bottomrule
%     % \bottomrule
%     \end{tabular}
%     }
% \end{wraptable} 

% \ml{Do we need to show the DFT explicitly? A theorem for the across block encoding.}
% \paragraph{High-level idea}
% As analyzed in Section~\ref{subsec:motiv}, a block circulant GEMM can be decomposed into two steps: a circulant GEMM within each block and a general GEMM across blocks. Simply using one of SIMD encoding or coefficient encoding cannot be fully compatible with it, we propose to embrace the strengths of both SIMD and coefficient encoding schemes. Specifically, we leverage coefficient encoding within each circulant block and utilize SIMD encoding across circulant blocks.
% We find that a block circulant matrix multiplication can be decomposed into two steps: \textbf{\underline{1)}} circulant matrix multiplication within each block, and \textbf{\underline{2)}} general matrix multiplication between blocks when we consider each block as a basic unit. For \textbf{\underline{1)}}, since circulant matrix multiplication corresponds to 1-D convolution, we can employ coefficient encoding to achieve the desired output by carefully designing the encoding methods. For \textbf{\underline{2)}}, as it is converted into general matrix multiplication, we can utilize SIMD encoding to reduce the number of rotations. Thus, it allows us to harness the strengths of both SIMD and coefficient encoding schemes.
% \paragraph{Encode within a circulant block $\operatorname{CirEncode}_{in}$}
% Previous works Cheetah~\cite{huang2022cheetah} and Iron~\cite{hao2022iron} design the coefficient encoding methods for GEMM. However, they both suffer from two drawbacks: \textbf{\underline{1)}} low coefficient utilization rate. As shown in Section 3.1 in Cheetah~\cite{huang2022cheetah} and Section 4.1 in Iron~\cite{hao2022iron}, the output polynomial coefficient utilization rate is only $\frac{1}{d_2}$, resulting in significant communication cost. \textbf{\underline{2)}} Inconsistent input and output packing, hindering us from consecutively computing on the output.
% In this work, overcoming these limitations, we build $\operatorname{CirEncode}_{in}$ for a circulant GEMM. $\operatorname{CirEncode}_{in}$ possesses two key properties: \textbf{\underline{1)}} $100\%$ coefficient utilization without any wastage. \textbf{\underline{2)}} Consistent packing of inputs and outputs, which is crucial for layer fusion in Section~\ref{sec:fusion}. Figure~\ref{fig:cirencode} illustrates a toy example of $\operatorname{CirEncode}_{in}$.\footnote{$\operatorname{CirEncode}_{in}$ uses $\operatorname{mod} x^n-1$ which is slightly different from~\cite{huang2022cheetah}, we justify this choice in Appendix~\ref{app:cyclic_nega_cyclic}.} 
% % We first treat each row of $X$ as a unit, that is, encoding a row consecutively. Then we employ polynomial modular multiplication to produce the desired output $\hat{y}$. 
% Formally, we define two encoding functions $\pi_\mathrm{X}: \mathbb{Z}^{d_1\times b}\rightarrow \mathbb{A}_n$ and $\pi_\mathrm{W}: \mathbb{Z}^{b\times b}\rightarrow \mathbb{A}_n$ as follows: \ml{dimension not correct}
% \begin{align*}
%     & \hat{x}=\pi_{\mathrm{X}}({X}) \quad \mathrm{s.t.} \quad \hat{x}[id_1+j]=X[i,j],i\in [d_1], j\in [b]\\
%     & \hat{w}=\pi_{\mathrm{W}}({W}) \quad \mathrm{s.t.}\quad \hat{w}[id_1]=W[i,0], i\in [b]
% \end{align*}
% where other coefficients of $\hat{w}$ are set to 0. Multiplication of polynomials $\hat{y}=\hat{w}\times \hat{x}$ directly gives the result of ${Y}={WX}$ as described in Theorem~\ref{theorem:encode} and we defer the proof to Appendix~\ref{proof:encode}.

% \begin{theorem}\label{theorem:encode}
%     Assuming $bd_1\le n$ and given two polynomials $\hat{x}=\pi_{\mathrm{X}}({X})$ and $\hat{w}=\pi_{\mathrm{W}}({W})$. The polynomial multiplication result $\hat{y}=\hat{w}\times \hat{x}$ directly maps to the result of ${Y}={WX}\in \mathbb{Z}^{b\times d_1}$ where ${Y}[i,j]=\hat{y}[id_1+j]$.
% \end{theorem}

% \paragraph{Encode across circulant blocks $\operatorname{CirEncode}_{out}$}
% We first consider each circulant block as a basic unit and transform the block circulant GEMM into GEMM with dimension $(d_1,\frac{d_2}{b},\frac{d_3}{b})$. Consequently, we can apply SIMD encoding to encode the input and weight matrices following~\cite{pang2023bolt} and use a DFT to transform $\operatorname{CirEncode}_{in}$ into $\operatorname{CirEncode}_{out}$ for each block. Similar to Lemma~\ref{lemma:DFT}, the correctness is given by: $\lj \operatorname{DFT}(x) \rj_{\operatorname{CirEncode}_{out}}\odot \lj \operatorname{DFT}(w) \rj_{\operatorname{CirEncode}_{out}}=\lj x \rj_{\operatorname{CirEncode}_{in}}\times \lj w \rj_{\operatorname{CirEncode}_{in}}$ .
% % \begin{equation*}
% %     \operatorname{DFT}(\lj \cdot \rj_{\operatorname{CirEncode}_{in}})\odot \operatorname{DFT}(\lj \cdot \rj_{\operatorname{CirEncode}_{in}})=\operatorname{DFT}(\lj \cdot \rj_{\operatorname{CirEncode}_{in}}\times \lj \cdot \rj_{\operatorname{CirEncode}_{in}})
% % \end{equation*}
% % \xts{do we need this??}Our experiment shows that the latency of plaintext DFT can be ignored compared to HE operations.
% Furthermore, we extend the BSGS strategy~\cite{pang2023bolt} to~\encode~to reduce the number of rotations with details in Appendix~\ref{app:cirencode}. In addition to matrix multiplication, we also design~\encode~to convolution operations, with further details provided in Appendix~\ref{app:encode_conv} due to space constraints.


\begin{table}[!tb]
    \renewcommand{\arraystretch}{1.0}\
    \Huge
    \centering
    \caption{Complexity comparison with previous works. The data is measured with dimension $(d_1,d_2,d_3)=(512,768,3072)$, the polynomial degree $n=8192$ and block size $b=8$.}
    \label{tab:complexity_compare}
    \resizebox{0.7\linewidth}{!}{
    \begin{tabular}{c|cccc}
    \toprule 
    % \toprule
    \multirow{1}{*}{Framework}  &  \multicolumn{1}{c}{\# HE-Pmult}&\# HE-Rot & \# Input & \# Output\\
    \midrule
    \multirow{2}{*}{CrypTFlow2~\cite{rathee2020cryptflow2}}& $O(d_1d_2d_3/n)$ &$O(d_1(d_2+d_3)/n+d_3)$&$O(d_1d_2/n)$ & $O(d_1d_3/n)$\\
     &147456&3312&18 MB&24 MB \\
    \midrule
    \multirow{2}{*}{Cheetah/Iron~\cite{huang2022cheetah,hao2022iron}$^{\mathrm{*}}$}& $O(d_1d_2d_3/n)$ &\multirow{2}{*}{0} &$O(d_1d_2/n)$ & $O(d_1d_2d_3/n)$\\
    & 147456 & & 18 MB & 334 MB \\
    \midrule
    % \multirow{1}{*}{Iron}& $\frac{HWCKR^2}{N}$ &\multirow{2}{*}{0} &$\frac{HWCR^2}{N}$&$K\lceil \frac{HWR^2}{N}\rceil $\\
    % ~\cite{hao2022iron}&384&&0.11 MB&21.77 MB \\
    % \hline
    \multirow{2}{*}{Bumblebee~\cite{lu2023bumblebee}}& $O(d_1d_2d_3/n)$ &$O(\lceil d_1/n\rceil d_3)$  &$O(d_1d_2/n)$ & $O(d_1d_3/n)$\\
    & 147456 & 3072 &18 MB&24 MB \\
    % +tile&384&48&0.88 MB&0.68 MB \\
    \midrule
    \multirow{2}{*}{Neujeans/Bolt~\cite{ju2023neujeans,pang2023bolt}}& $O(d_1d_2d_3/n)$ &$O(d_2)$  &$O(d_1d_2/n)$ & $O(d_1d_3/n)$\\
    & 147456 & 720 &18 MB&24 MB   \\
    \multirow{2}{*}{Bolt+BSGS}& $O(d_1d_2d_3/n)$ &$O(\sqrt{d_1d_2d_3/n})$  &$O(d_1d_2/n)$ & $O(d_1d_3/n)$\\
    & 147456 & 528 &18 MB&24 MB \\
    % \hline
    % \multirow{1}{*}{Circulant}& $\frac{HW\max{(R^2C,K)}}{N}$ &\multirow{2}{*}{0}&$\frac{HWCR^2}{N}$&$\frac{HWK}{N}$\\
    % (Ours)&6&&0.11 MB&0.68 MB  \\
    \midrule
    \multirow{2}{*}{\encode~(ours)}& $O(d_1d_2d_3/(nb))$ &$O(\sqrt{d_1d_2d_3/(bn)})$  &$O(d_1d_2/n)$ & $O(d_1d_3/n)$\\
    &18432& 48 &18 MB&24 MB  \\

    % \multirow{2}{*}{+BSGS}& $O(d_1d_2d_3/(nb))$ &$O(\sqrt{d_1^2d_2^2d_3/(bn^2)})$  &$O(d_1d_2/n)$ & $O(d_1d_3/n)$\\
    % &48&4&0.11 MB&0.68 MB  \\
    \bottomrule
    \multicolumn{5}{c}{$^{\mathrm{*}}$We use cheetah's $1\times 1\ \operatorname{convolution}$ protocol whose cost is the same as Iron's $\operatorname{matmul}$ protocol.} 
    % \bottomrule
    \end{tabular}
    }
\end{table}

\begin{minipage}{0.48\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figs/breakdown.pdf} 
\end{minipage}
\hspace{3mm}
\begin{minipage}{0.48\textwidth}
    \centering
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{c|c|cccc}
    \toprule 
    % \toprule
    \multirow{2}{*}{Method}& \multirow{2}{*}{\makecell{Sparsity/\\ Block size}} &\multicolumn{4}{c}{Number of rotations left (\%) $\downarrow$}\\
    \cmidrule{3-6}
    & & MBV2& ViT& ViT-Tiny& Average\\
    \midrule
    \multirow{3}{*}{\makecell{SpENCNN\\ \cite{spencnn}}}& 50\% &100 &100 &100 &100\\\
    & 75\% &99.36 &97.85 &99.26 &98.82\\
    & 87.5\% &92.96 &97.85 &99.26 &96.69\\
    \midrule
    \multirow{3}{*}{\makecell{\method\\ (ours)}}& b=2 &60.98 &65.25 &61.75 &\textbf{62.66}\\
    & b=4 &35.23 &41.92 &36.32 &\textbf{37.82}\\
    & b=8 &21.05 &27.70 &19.02 &\textbf{22.59}\\
    % \multirow{2}{*}{+BSGS}& $O(d_1d_2d_3/(nb))$ &$O(\sqrt{d_1^2d_2^2d_3/(bn^2)})$  &$O(d_1d_2/n)$ & $O(d_1d_3/n)$\\
    % &48&4&0.11 MB&0.68 MB  \\
    \bottomrule
    % \bottomrule
    \end{tabular}
    }
\end{minipage}\\
\begin{minipage}[t]{.48\textwidth}\centering%caption宏包
    \captionof{figure}{Latency breakdown of~\method~(b8) on MobileNetV2 and ViT.}
    \label{fig:exp_breakdown}
    \end{minipage}\hspace{3mm}%
\begin{minipage}[t]{.48\textwidth}\centering%
    \captionof{table}{Compared with SpENCNN in the number of rotations left. \ml{Not sure how useful this table is.}}
    \label{tab:exp_cmp_spencnn}
\end{minipage}



\subsection{Proof of Theorem~\ref{theorem:encode_across}}\label{proof:encode_across}
\textbf{Cyclic and Nega-cyclic convolutions.}
To prove Theorem~\ref{theorem:encode_across}, we first introduce the concepts of the cyclic and nega-cyclic convolutions. Within each circulant block,~\encode~operates over the ring $\mathbb{A}_n=\mathbb{Z}[x]/(x^n-1)$ in which a polynomial multiplication implements a cyclic convolution. While in the ring $\mathbb{A'}_n=\mathbb{Z}[x]/(x^n+1)$, a polynomial multiplication implements a nega-cyclic convolution. Both cyclic and nega-cyclic convolutions can be converted into element-wise modular multiplication through cyclic DFT and nega-cyclic DFT, respectively~\cite{longa2016speeding,ju2023neujeans}. Hence, following~\cite{longa2016speeding,ju2023neujeans}, we have Lemma~\ref{lemma:cyclic_DFT}.
\begin{lemma}
    \label{lemma:cyclic_DFT}
    $\operatorname{Cyclic\ DFT}(\hat{w})\odot \operatorname{Cyclic\ DFT}(\hat{x})=\operatorname{Cyclic\ DFT}(\hat{w}\times \hat{x})$ where $\hat{w},\hat{x},\hat{w}\times \hat{x} \in \mathbb{A}_n$.
\end{lemma}
Therefore, given $k$ circulant weight matrices $W_1, \ldots, W_k \in \mathbb{Z}^{b\times b}$ and input matrices $X_1, \ldots, X_k \in \mathbb{Z}^{b\times d_1}$, define the following polynomials $\hat{w}_i=\pi_{\mathrm{W}}({W_i})$ and $\hat{x}_i=\pi_{\mathrm{X}}({X_i})$ with $i \in [k+1]$. We have:
\begin{equation}\label{eq:proof_across}
\begin{aligned}
    &\lj \operatorname{DFT}(\hat{w}_0)|\ldots|\operatorname{DFT}(\hat{w}_{m-1})\rj_{\mathrm{SIMD}}\times \lj \operatorname{DFT}(\hat{x}_0)|\ldots|\operatorname{DFT}(\hat{x}_{m-1})\rj_{\mathrm{SIMD}}\\
    &=\lj \operatorname{DFT}(\hat{w}_0)\odot \operatorname{DFT}(\hat{x}_0)| \ldots | \operatorname{DFT}(\hat{w}_{k-1})\odot \operatorname{DFT}(\hat{x}_{k-1})\rj_{\mathrm{SIMD}}\\
    &=\lj \operatorname{DFT}(\hat{w}_0\times \hat{x}_0)|\ldots |\operatorname{DFT}(\hat{w}_{k-1}\times \hat{x}_{k-1})\rj_{\mathrm{Coeff}} \\
    &=\lj\operatorname{DFT}(\hat{y}_0)|\ldots |\operatorname{DFT}(\hat{y}_{k-1})\rj_{\mathrm{Coeff}} \\
\end{aligned}
\end{equation}
In Equation~\ref{eq:proof_across}, all instances of DFT refer to the cyclic DFT. The second line follows directly from Lemma~\ref{lemma:cyclic_DFT} while the last line is derived from Theorem~\ref{theorem:encode}. Through Equation~\ref{eq:proof_across}, we simultaneously evaluate $k$ circulant GEMMs with dense encoding.

\encode~applies SIMD encoding across circulant blocks, operating over $\mathbb{A'}_n$. However, the correctness of Equation~\ref{eq:proof_across} can still be guaranteed based on the following facts: \textbf{\underline{1)}} After performing the cyclic DFT, we obtain $\operatorname{DFT}(\hat{w}_1)$ and $\operatorname{DFT}(\hat{x}_1)$, etc. The next step requires element-wise modular multiplication to compute $\operatorname{DFT}(\hat{w}_1)\odot \operatorname{DFT}(\hat{x}_1)$. Thus, the correctness is maintained as long as the implementation can perform element-wise modular multiplication, regardless of the internal implementation. \textbf{\underline{2)}} In SIMD encoding, element-wise multiplication is implemented through a polynomial multiplication in the coefficient domain, requiring nega-cyclic iDFT/DFT, as shown in Figure~\ref{fig:cntt}. Consequently, the modulus of the nega-cyclic iDFT/DFT must match the modulus of the cyclic DFT to avoid overflow error. Fortunately, both cyclic DFT and nega-cyclic DFT can use the same modulus, as cyclic DFT can be transformed into nega-cyclic DFT via a linear transformation~\cite{longa2016speeding}. Therefore, to guarantee correctness, we employ the same modulus for both cyclic DFT and nega-cyclic iDFT/DFT in~\encode~as we illustrate in Figure~\ref{fig:cntt}.
\begin{figure}[!tb]
    \centering
    \includegraphics[width=1.0\linewidth]{figs/cntt.pdf}
    \caption{The correctness of~\encode.}\label{fig:cntt}
\end{figure}


